Audit Games with Multiple Defender Resources

Modern organizations (e.g., hospitals, social networks, government agencies) rely heavily on audit to detect and punish insiders who inappropriately access and disclose confidential information. Recent work on audit games models the strategic interaction between an auditor with a single audit resource and auditees as a Stackelberg game, augmenting associated well-studied security games with a configurable punishment parameter. We significantly generalize this audit game model to account for multiple audit resources where each resource is restricted to audit a subset of all potential violations, thus enabling application to practical auditing scenarios. We provide an FPTAS that computes an approximately optimal solution to the resulting non-convex optimization problem. The main technical novelty is in the design and correctness proof of an optimization transformation that enables the construction of this FPTAS. In addition, we experimentally demonstrate that this transformation significantly speeds up computation of solutions for a class of audit games and security games.

==> Constraint.tex <==
The definition of the constraints set $C$ provides an algorithm to construct the set.
However, as discussed earlier, that algorithm is always exponential. We 
provide an alternate algorithm to find constraints in $C$ and sufficient
condition under which the number of constraints is polynomial in number.
First, the following counterexample reveals that in the worst case the number of constraints in $C$ will be super-polynomial. Consider $k$ resources $s_1, \ldots, 
s_k$ and $2k$ targets $t_1, \ldots, t_{2k}$. Each resource $s_i$ can inspect targets
$t_1, \ldots, t_{2i}$. Consider any set of $k$ targets formed by picking target pairs
$t_{2i-1}, t_{2i}$ for all possible $i$, except $i=1$. The number of such sets are $k-1 \choose k/2$.
Each such set of target results in a valid constraint, since the number of targets 
that can audit these targets in less than $k$. This is because the first resource only
inspects $t_1, t_2$, and that pair is never chosen. Thus, we get $k-1 \choose k/2$
constraints, which is clearly not polynomial.

The intuition behind the alternate algorithm is that instead of iterating over sets of inspection resources, we could iterate over sets of targets. As a first step, we identify similar targets and merge them. More precisely,
any targets that can be audited by the exact same set of inspections are equivalent. Then, the algorithm
to determine constraints is described in Algorithm~\ref{alg2}.
\begin{algorithm}[h] \label{alg2}
\DontPrintSemicolon
Compute $F$, the map from $T$ to $2^{\{s_1, \ldots, s_k\}}$ using $R$.\;
Let $PV(t)$ be the probability variable $p_t$ for target $t$\;
Merge targets with same $F(T)$ to get set $T'$ and map $W$, with $W(t')$ the no. of merged targets that yielded $t'$\;
Let $PV(t')$ be the set of probability variables associated with $t'$\;
Form an intersection graph $G$ with nodes $t' \in T'$ and each node denoting set $F(T')$\;
$L \leftarrow \mathsf{CONNECTEDSUBGRAPH}(G)$ \;
$C \leftarrow \phi$\;
\For{$l \in L$}{
	Let $V$ be all the vertices on $l$ \;
	$P \leftarrow \cup_{v \in V} PV(v)$\;
	$k \leftarrow \sum_{v \in W} W(t')$\;
	\If{$|P| > k$}{
		$C \leftarrow C \cup \{\sum_{p \in P} p \leq k\}$
	}
}
\Return $C$\;
\caption{$\mathsf{CONSTRAINT\_FIND}(T, K, R)$}
\end{algorithm}

%In the above algorithm we treat paths as walks with no repeating edges. Note that we do 
%not use simple paths. 
The algorithm builds an intersection graph from the merged target, i.e., treat every merged target as a node and two 
nodes are linked if the two set of inspection resources corresponding to the 
nodes intersect. Then, the algorithm iterates through every connected induced
sub-graph and builds constraints from the targets associated with the 
nodes in the sub-graphs and the set of inspection resources associated with them.

Next, we proof the correctness of the Algorithm~\ref{alg2}. After that, 
we investigate the conditions under which the Algorithm~\ref{alg2} runs efficiently, and yields a polynomial sized $C$.

\paragraph{Correctness of $\mathsf{CONSTRAINT\_FIND}$.}
The correctness of Algorithm~\ref{alg2} requires us to show that the output of the naive
algorithm (iterating over all subsets of resources) is the same as $\mathsf{CONSTRAINT\_FIND}$.
Assume constraint $c$ is in the output of the naive algorithm. Restrict the constraint $c$ 
to be a non-implied constraint, i.e., $c$ cannot be written as the sum of two or more
other constraints in $C$. Note that such a restriction does not change the region defined by
the set $C$. By the description of the 
naive algorithm, this constraint must correspond to a set of inspections, say $S$, and
the set of targets $T_S$ inspected only by inspections in $S$, and there exists
no subset of $T_S$ and $S$ such that the subset of targets is inspected only by the subset of inspections. The constraint $c$ is of the form $P(T_S) \leq |S|$, where $P(T_S)$ is the 
sum of the probability variables for targets in $T_S$. Now, for the intersection graph
representation, every node $x$ represents targets that are inspected by a given subset $x_s$ of inspections. For our case, we claim that every $t \in T_S$ is either equivalent to or linked to another target in $T_S$, otherwise 
we have the subset $\{t\} \subset S$ inspected only by $t_s \subset T_S$. Thus, the 
targets in $T_S$ form a connected induced sub-graph. Thus, we conclude that the 
$\mathsf{CONSTRAINT\_FIND}$ algorithm will consider this set of targets and find the
non-implied constraint $c$.

Next, assume that $\mathsf{CONSTRAINT\_FIND}$ finds a constraint $c$. As this
corresponds to a connected induced sub-graph (with targets as nodes), we obtain a set of targets 
$T$ and a set of inspections $\cup_{t \in T} F(t)$ such that targets in $T$ are audited
by $\cup_{t \in T} F(t)$ only. Thus, by definition of the construction of $c$, this constraint
is same as the constraint $c'$ obtained by the naive algorithm when it considers the set
$\cup_{t \in T} F(t)$. That is, $c$ will also be found by the naive algorithm.

\paragraph{Conditions for efficient $\mathsf{CONSTRAINT\_FIND}$.} The algorithm 
$\mathsf{CONSTRAINT\_FIND}$ is clearly not polynomial time in the worst case
because of the iteration over all connected sub-graphs. We state here sufficient conditions
for $\mathsf{CONSTRAINT\_FIND}$ to be polynomial. These conditions also
correspond to natural setting in real auditing scenarios; we discuss this later in 
Section~\ref{}

\begin{itemize}
\item Graphs with $O(\log n)$ nodes. The maximum number of connected induced subgraphs in 
graph with $t$ nodes is $2^t$ (take any subset of vertexes). Thus, clearly a graph with
$O(\log n)$ nodes will have polynomially many connected sub-graphs.
\item Graphs with constant max degree and constant number of nodes with degree $\geq 3$. The number of connected induced subgraphs in a 
tree with max degree $d$ and $t$ vertexes with degree $\geq 3$ is bounded from above 
by $2^{(2(d+1))^{t+1}} n^{(d+1)^{t+1}}$. To prove this, denote by $T(n,d,t)$ the worst case number of connected 
induced sub-graphs in a graph with $n$ vertices, and max degree $d$ and $t$ vertices with degree $\geq 3$. 

Remove a vertex $X$ with degree $\geq3$, to get $k \leq d$ disconnected 
components. Each connected sub-graph in any component, that was linked to $X$, could be combined with any connected sub-graph of any other component linked to $X$, yielding a new connected sub-graph. 
%Note that for any 
%connected sub-graph that was linked to $X$ in any component, there is another 
%connected sub-graph that was not linked to $X$ in that component (remove the vertex 
%that linked to $X$ from the sub-graph). Thus, the number of connected sub-graph that 
%was linked to $X$ in any component can be upper bounded by $T(n-1,d,t-1)/2$.
Thus, considering every subset of the $k$ components, we get
$$
T(n,d,t) \leq 2^k \left(T(n-1, d, t-1)\right)^k 
$$
Observing that $k < d+1$, and $T(n-1, d, t-1) \leq T(n, d, t-1)$ we get
$$
T(n,d,t) \leq \left( 2T(n, d, t-1) \right)^{d+1}
$$
Thus, we see that $T(n,d,t) = 2^{(2(d + 1))^{t+1}}(n)^{(d + 1)^{t+1}}$ satisfies the above equation. 

As part of the induction, the base case requires reasoning about a graph with max degree either $1$ or $2$
($t = 0, d = 1$ or $2$). Thus, we need to show that the connected sub-graphs is less than $n^{d+1}$, which is $n^2$ for max-degree $1$ and $n^3$ for max-degree $2$.
The max-degree $1$ case is trivial. For the max-degree $2$ case, such graphs can be decomposed into paths and cycles, and the number of connected sub-graphs
on cycles and paths is less that $n^2$.
%\item Bound on number of nodes with degree $\geq 3$.
\end{itemize}

==> Optimization.tex <==

We present a
FPTAS under the condition that the set $C$ has polynomially many constraints.



\paragraph{FPTAS.} Our algorithm builds on an earlier algorithm for a restricted auditing 
scenario~\cite{}. We solve the problem after extracting constraints $C$, thus, the variables
in our problem are just $p_i$'s. The final solution involves computing feasible values of
$p_i^j$'s (this can be done in polynomial time since it is a linear feasibility problem), followed
by the B-VN decomposition (see details shown in Section~\ref{}) to obtain the distribution
over pure allocations.

First, we simplify our problem $P_*$ by eliminating variables $p_i^j$ and introducing constraints in $C$, and (wlog) letting $*$ be $n$.
$$
\begin{array}{llc}
\displaystyle\max_{p_{i},x} & p_{n}U^a_D (t_n) + (1 - p_{n})U^u_D (t_n) - ax \ ,&\\
\mbox{subject to}& \forall i \neq n. \ p_{i}(U^a_A (t_i) -x) + (1 - p_{i})U^u_A (t_i) & \\
%&  \forall i \neq *. \ p_{i}(U^a_A (t_i) -x) + (1 - p_{i})U^u_A (t_i)  &\\
&  \ \ \ \ \ \ \ \ \ \
\leq p_{*}(U^a_A (t_n) - x) + (1 - p_{n})U^u_A (t_n)  \ ,&\\
& \forall i.  \ 0 \leq p_i \leq 1 \ , \ \ \ \ \ 0 \leq x \leq 1 \ , \\
& c \in C \ .
\end{array}
$$
We rewrite $P_{n}$ 
in a more compact form.
Let 
$\Delta_{D,i} = U^a_D (t_i)  - U^u_D (t_i)$, $\Delta_{i} = 
U^u_A (t_i) - U^a_A (t_i)$ and $\delta_{i,j} = U^u_A (t_i) - U^u_A (t_j)$.
$\Delta_{D, i}$ and $\Delta_{i}$ are always positive, and
 $P_n$ reduces to:
 
$$
\begin{array}{llc}
\displaystyle\max_{p_{i},x} & p_{n} \Delta_{D,n} - ax \ ,&\\
\mbox{subject to}& \forall i \neq n. \ p_i (-x - \Delta_i) + p_n (x + \Delta_n) + \delta_{i,n}  \leq 0 & \\
%&  \forall i \neq *. \ p_{i}(U^a_A (t_i) -x) + (1 - p_{i})U^u_A (t_i)  &\\
%&  \ \ \ \ \ \ \ \ \ \ \leq p_{*}(U^a_A (t_n) - x) + (1 - p_{n})U^u_A (t_n)  \ ,&\\
& c \in C, \ \ \forall i.  \ 0 \leq p_i \leq 1 \ , \ \ \ 0 \leq x \leq 1 \ .
\end{array}
$$

\textit{Property of an optimal point.} First, observe that the quadratic inequality can
be rewritten as $$
\frac{p_n (x + \Delta_n) + \delta_{i,n}}{x + \Delta_i} \leq p_i \ .
$$ 
Suppose $p_i^*$'s and $x^*$ is an optimal point, and suppose for some $j$ we have the
strict inequality
$$
\frac{p_n^* (x^* + \Delta_n) + \delta_{j,n}}{x^* + \Delta_j} < p_j^* \ .
$$
Let $p_j' = \min(0, \frac{p_n^* (x^* + \Delta_n) + \delta_{j,n}}{x^* + \Delta_j})$. Then, 
we claim that $p_1^*, \ldots, p^*_{j-1}, p_j', p^*_{j+1}, p^*_n, x^*$ is also an optimal point.
This is easy to see, since, decreasing $p_j$ is not restricted by any inequality other than
the quadratic inequality and the objective only depends on $p_n$. As a result, we 
can restrict the problem to be equalities for all the quadratic constraints.

\textit{Decomposing into sub-problems.} Then, 
similar to an earlier paper~\cite{}, we sort $\delta_{i,n}$'s to get a sorted array 
$\delta_{(i),n}$ in ascending order. Then, split the optimization
problem $P_n$ into sub-problems $EQ_{(j)}$, where in each problem $EQ_{(j)}$ it is assumed that 
$p_n, x$ lies between the hyperbolas $p_n (x + \Delta_n) + \delta_{(j),n}$ (open 
boundary) and $p_n (x + \Delta_n) + \delta_{(j+1),n}$ (closed boundary) in the plane 
spanned by $p_n, x$. Thus, in $EQ_{(j)}$, $p_n 
(x + \Delta_n) + \delta_{(j),n}$ is non-negative
for all $(k) > (j)$ and negative otherwise. For the negative case, using the property
of the optimal point above, we claim that for all $(k) \leq (j)$ we can set $p_{(k)} = 0$.
The optimal value for $P_n$ can be found
by solving each $EQ_{(j)}$ and taking the best solution from these sub-problems.

The optimization problem for $EQ_{(j)}$ :
 $$
\begin{array}{llc}
\displaystyle\max_{p_{i},x} & p_{n}\Delta_{D,n} - ax \ ,&\\
\mbox{subject to}& \forall (i) > (j). \ 0 \leq \frac{p_n (x + \Delta_n) + \delta_{(i),n}}{x + \Delta_{(i)}} = p_{(i)} \leq 1 & \\
& p_n (x + \Delta_n) + \delta_{(j),n} < 0 &\\
& p_n (x + \Delta_n) + \delta_{(j+1),n} \geq 0 &\\
%&  \forall i \neq *. \ p_{i}(U^a_A (t_i) -x) + (1 - p_{i})U^u_A (t_i)  &\\
%&  \ \ \ \ \ \ \ \ \ \ \leq p_{*}(U^a_A (t_n) - x) + (1 - p_{n})U^u_A (t_n)  \ ,&\\
& \forall (i) \leq (j).  \ p_{(i)} = 0 \ , \ \ \ \ \ 0 \leq x \leq 1 \\
& c \in C \ .
\end{array}
$$
As no $p_i$ (except $p_n$) shows up in the objective, and due to the equality constraints
on particular $p_i$'s, we can replace those $p_i$'s by function of $p_n, x$. 
Other $p_i$'s are zero. Then, denote by $c(p_n, x)$ the inequality
obtained after substituting $p_i$ with the function of $p_n, x$ (or zero) for constraints
$c \in C$. Thus, we get the 
following two variable optimization problem
 $$
\begin{array}{llc}
\displaystyle\max_{p_{i},x} & p_{n}\Delta_{D,n} - ax \ ,&\\
\mbox{subject to}& \forall (i) > (j). \ \frac{p_n (x + \Delta_n) + \delta_{(i),n}}{x + \Delta_{(i)}} \leq 1 & \\
& p_n (x + \Delta_n) + \delta_{(j),n} < 0 &\\
& p_n (x + \Delta_n) + \delta_{(j+1),n} \geq 0 &\\
%&  \forall i \neq *. \ p_{i}(U^a_A (t_i) -x) + (1 - p_{i})U^u_A (t_i)  &\\
%&  \ \ \ \ \ \ \ \ \ \ \leq p_{*}(U^a_A (t_n) - x) + (1 - p_{n})U^u_A (t_n)  \ ,&\\
& 0 \leq p_n \leq 1 \ , \ \ \ 0 \leq x \leq 1 \\
& c(p_n, x) \in C \ .
\end{array}
$$
Observe that we removed the $0 \leq$ condition in first set of constraints because that is 
implied by the next two constraints. Next, note that any constraint (indexed by $b$) with two 
variables $p_n, x$ can be expressed as $p_n \leq f_b(x)$ (closed boundary) 
for constraint specific ratio of polynomials $f_b(x)$ or by 
$p_n < \frac{-\delta_{(j),n}}{x + \Delta_n}$ (open boundary). However, we close the
open boundary, i.e., $p_n \leq \frac{-\delta_{(j),n}}{x + \Delta_n}$, and solve the 
problem, and returning an infeasible solution in case the solution is on the boundary
$p_n = \frac{-\delta_{(j),n}}{x + \Delta_n}$. This is justified by the fact that the curve
$p_n = \frac{-\delta_{(j),n}}{x + \Delta_n}$ is included in the other optimization 
problem $EQ_{(j-1)}$, and would be output by that sub-problem if it indeed is the 
global maximizer. Thus, we represent the optimization problem as
 $$
\begin{array}{llc}
\displaystyle\max_{p_{i},x} & p_{n}\Delta_{D,n} - ax \ ,&\\
\mbox{subject to}& \forall b \in \{1, \dots,  B\}. ~ p_n \leq f_b(x) & \\
%& p_n (x + \Delta_n) + \delta_{(j),n} < 0 &\\
%& p_n (x + \Delta_n) + \delta_{(j)+1,n} \geq 0 &\\
%&  \forall i \neq *. \ p_{i}(U^a_A (t_i) -x) + (1 - p_{i})U^u_A (t_i)  &\\
%&  \ \ \ \ \ \ \ \ \ \ \leq p_{*}(U^a_A (t_n) - x) + (1 - p_{n})U^u_A (t_n)  \ ,&\\
& \ 0 \leq p_n \leq 1 \ , \ \ \ 0 \leq x \leq 1 \ ,
\end{array}
$$
where $B$ is the total number of constraints described as above. 

\textit{Solving sub-problem.} We first claim that it is easy to solve the problem with $p_n 
=1$ or $p_n=0$ and $x=0$ or $x=1$. The fixed $x$ case is obvious, since the problem 
is a linear program for fixed $x$. The fixed $p_n$ case is equivalent to minimizing
$x$ with constraints that are of the form $f(x) \leq0$, where $f$ is a polynomial in $x$. 
For any polynomial constraint, it is possible to obtain roots of the polynomial and hence 
find the intervals of $x$ that satisfies the constraint. Doing so for the polynomially many constraints and finding the intersection of intervals yields the minimum value of $x$ that
satisfies all constraints. 

Next, we claim that the optimal point cannot be an interior
point of the region defined by the constraints i.e., it cannot
be the case that all such inequalities are strict for the optimal point.  We can derive an 
easy contradiction for this scenario. Assume $p_n^*, x$ is optimal.
As $f_b$ is continuous in $x$, if all inequalities are strict, then it is possible to 
increase the value of optimal $p_n^*$ by a small amount, without violating the 
constraints. Clearly, this increased value of $p_n$ results in a higher objective value,
contradicting the assumption that $p_n^*, x^*$ is optimal.

Hence, given the above claims, the procedure in Algorithm~\ref{alg1} finds the maximum of the 
optimization under consideration. 

\begin{algorithm}[h] \label{alg1}
\DontPrintSemicolon
Solve the problem for $p_n= 0,1$ and $x = 0,1$\; 
Collect solutions $(p_n, x)$ from the above in $M$\;
\For{$b \leftarrow 1$ \KwTo $B$}{
	Replace $p_n = f_b(x)$ in the objective to get $F(x) = f_b(x)\Delta_{D,n} - ax$ \;
	Take the derivative to get $F'(x) = \frac{\partial F(x)}{\partial x}$\;
	$R \leftarrow \mathsf{ROOTS}(F'(x), 2^{-l}, (0,1))$\;
	$R' \leftarrow \mathsf{MAKEFEASIBLE}(R)$\;
	From $R'$ obtain set $M'$ of potential solutions $(p_n, x)$\;
	$M \leftarrow M \cup M'$\;
}
\For{$(b,b') \in \left\{(b,b') ~|~ b \in B, b \in B, b' > b \right\}$}{
	Equate $f_b(x) = f_{b'}(x)$ to get $F(x) = 0$ \;
	$R \leftarrow \mathsf{ROOTS}(F(x), 2^{-l}, (0,1))$\;
	$R' \leftarrow \mathsf{MAKEFEASIBLE}(R)$\;
	From $R$ obtain set $M'$ of potential solutions $(p_n, x)$\;
	$M \leftarrow M \cup M'$\;
}
$(p_n^*, x^*) \leftarrow \arg\max_{M} \{ p_n \Delta_{D,n} - ax \}$ \;
\Return $(p_n^*, x^*)$
\caption{$\mathsf{APX\_SOLVE}(l, EQ_{(j)})$}
\end{algorithm}
Algorithm~\ref{alg1} first searches the maximizer on the boundaries (in the first loop)
and then searches the maximizer at the intersection of two boundaries (second loop).
The roots are found to an additive approximation factor of $2^{-l}$ and similar
to an earlier approach~\cite{}, the case of roots lying outside the feasible region (due
to approximation) is taken care of by function $\mathsf{MAKEFEASIBLE}$.
